PT-Spike: A Precise-Time-Dependent Single Spike Neuromorphic Architecture with Efficient Supervised Learning

One of the most exciting advancements in AI over the last decade is the wide adoption of ANNs, such as DNN and CNN, in many real-world applications. However, the underlying massive amounts of computation and storage requirement greatly challenge their applicability in resource-limited platforms like the drone, mobile phone, and IoT devices etc. The third generation of neural network model--Spiking Neural Network (SNN), inspired by the working mechanism and efficiency of human brain, has emerged as a promising solution for achieving more impressive computing and power efficiency within light-weighted devices (e.g. single chip). However, the relevant research activities have been narrowly carried out on conventional rate-based spiking system designs for fulfilling the practical cognitive tasks, underestimating SNN's energy efficiency, throughput, and system flexibility. Although the time-based SNN can be more attractive conceptually, its potentials are not unleashed in realistic applications due to lack of efficient coding and practical learning schemes. In this work, a Precise-Time-Dependent Single Spike Neuromorphic Architecture, namely "PT-Spike", is developed to bridge this gap. Three constituent hardware-favorable techniques: precise single-spike temporal encoding, efficient supervised temporal learning, and fast asymmetric decoding are proposed accordingly to boost the energy efficiency and data processing capability of the time-based SNN at a more compact neural network model size when executing real cognitive tasks. Simulation results show that "PT-Spike" demonstrates significant improvements in network size, processing efficiency and power consumption with marginal classification accuracy degradation when compared with the rate-based SNN and ANN under the similar network configuration.

==> implem.tex <==
\section{Implementation}
\label{sec:implem}

for FPGA implementation. 3/4 column.
1. design diagram.
2. specs and parameters.
3. description.
Field Programmable Gate Array (FPGA) is known to be a capable platform for energy efficient design campared with CPU and GPU designs. In order to fully leverage the benefit of PT-Spike, we imeplent PT-Spike on a Xilinx Artix7-100 FPGA. 

The system is used to make MNIST classification. The system architecture is shown in Figure. There are three main functional modules. The Image Reader is used to read out image patterns and generate the spikes according to the image pattern to be classified. The Weight Reader is used to read out the weights of the spiking neural networks in accordence to the image pattern. The Processing Element takes the corresponding outputs from Image Reader and Weight Reader, and computes the result by vector multiplication, the result that exceeds the presetted threshold will indicted the classification result and terminate the computation for current image.

The performance of the FPGA design is a trade off between space and time, more computational resources mean faster processing time but higher in power consumption, while less computational resource mean longer processing time but lower in power consumption. In our reference FPGA design, we implemented one Processing Element which contains four multipliers in parallel, this configuration archieves decent processing time while maintains the hardware resources in a relatively small scale. Alternative configurations are possible. 

Table. showed the utilization of the logic resource of the reference design in Artix7-100. The Artix7-100 is medium in logic capacity, with this reference, PT-Spike exhibits good capability in logic efficency. For all the four logic primitives, the utilization Slice LUTs and Slice registers are less than 1\%, while the utilization of DSP Slices and Block RAMs are less than 3\%.

\begin{table}[]
\centering
\caption{Artix7-100 Logic Utilization}
\label{tbl_hb}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
Resources & \begin{tabular}[c]{@{}c@{}}Slice LUTs\end{tabular} & \begin{tabular}[c]{@{}c@{}}Slice Registers\end{tabular} & \begin{tabular}[c]{@{}c@{}}DSP Slices\end{tabular} & \begin{tabular}[c]{@{}c@{}}Block RAMs\end{tabular} \\ \hline\hline
Occupied & 498 & 817 & 4 & 7 \\ \hline
Total & 63400 & 126800 & 240 & 270 \\ \hline
Percentage & 0.79\% & 0.64\% & 1.67\% & 2.59\% \\ \hline
\end{tabular}
}
\end{table}

\begin{figure*}[hbpt]
\begin{centering}
\includegraphics[width=1\textwidth]{PTsch.pdf}
\end{centering}
\caption{%
\label{ptsch}
The schematic of the implemented FPGA design.
}
\end{figure*}





*evaluation and estimation for power, will be discussed soon*

==> related.tex <==
%\vspace{-6pt}
\section{Related Works}
\label{sec:rw}
%\vspace{-6pt}

\subsection{Neuromorphic Designs}
Seo et al.~\cite{seo201145nm} proposed a 45nm CMOS neuromorphic chip for ultra-dense, ultra-low power brain-like cognitive computing. 

Chu et al.~\cite{chu2015neuromorphic} proposed a memristor and leaky I\&F based meromorphic design for visual pattern recognition. 

However, these works mainly discuss the hardware implementation while the adopted benchmarks and the functionality of proposed neuromorphic designs are far away from the realistic cognitive tasks. 

Neil et al.~\cite{neil2014minitaur} and Liu et al.~\cite{liu2016memristor} proposed FPGA/memristor cross-bar based spiking neuromorphic designs by implementing the multilayer perceptron (MLP) to handle MNIST handwritten cognitive task. 

Cao et al.~\cite{cao2015spiking} and Esser et al.~\cite{esser2016convolutional} proposed spiking based deep convolutional neuromorphic designs to handle more complex realistic applications. 

However, these works are majorly focus on the neural network model mapping and hardware implementations but merely discuss the spiking model optimization, i.e. coding, decoding and learning approaches etc. In real-world applications, training of the rate-based SNN can be usually performed off-line by directly deploying the learning rules from artificial neural network (ANN)~\cite{neil2014minitaur, liu2016memristor, cao2015spiking, esser2016convolutional} due to the similarity between numerical information representation of ANNs and rate-based coding. However, the popular learning approaches such as Back-propagation~\cite{rumelhart1988learning} in ANN or rate-coded SNN are unable to handle precise-time-dependent information due to the fundamentally different neural processing. In this work, time based coding and neural processing has been leveraged in our ``\textit{PT-Spike''} design to offering fast and power efficient training and inference through a single spike for realistic cognitive applications.

\subsection{Temporal Coding and Learning}
Thorpe et al.~\cite{thorpe1990spike}, Kempter et al.~\cite{kempter1996temporal} and Butts et al.~\cite{butts2007temporal} explored and perfected the feasibilities of time based neural coding. The arrival time or delay of spars spike train has been utilized to present information. However, these works are theoretically focus on the biologically explanation of computational time based neuronal models.

Zhao et al.~\cite{zhao2016energy} proposed an encoding circuits to handle the time based coding however still sticking on the hardware implementation without the end-to-end connected spiking neuromorphic solution.

Yu et al.~\cite{yu2013precise} proposed a complete time-based spiking neural network design for handling MNIST task. However, their solution is not optimized for hardware based meromorphic system and the adopted temporal learning rule and methodology are unsuitable for real-work application due to the limited accuracy.

Legenstein et al.~\cite{legenstein2005can} and Sjostrom et al.~\cite{sjostrom2010spike} developed unsupervised spiking-time-dependent plasticity (STDP) learning rule, which is able to handle precise-time-dependent spiking thus to adjust the membrane potential through weighting efficacies. However, the neural network structure and synaptic computation will be exponentially increased due to the expensive convergence and clustering.

Gutig et al.~\cite{gutig2006tempotron} proposed ``Tempotron'' learning rule and Ponulak et al.~\cite{ponulak2005resume} proposed ``Remote Supervised Method (ReSuMe)'' learning rule use the teaching spike to adjust the desired spiking time for temporal learning. However, these theoretical approaches neither hardware-favorable nor applicable to handle complex patterns.

In this work, to develop a low cost and efficient temporal learning rule, ``PT-Learning'' is further augmented from the ``Tempotron'' learning by considering a synthesized contribution of the cost function and the hardware-favorable time-dependent kernel for weight updating. By integrating with proposed ``A-Decoding'', ``\textit{PT-Spike}'' can improve the learning efficiency and accuracy significantly.


